NeRF-LiDAR: Generating Realistic LiDAR Point Clouds with Neural Radiance Fields

Labeling LiDAR point clouds for training autonomous driving is extremely expensive and difficult. LiDAR simulation aims at generating realistic LiDAR data with labels for training and verifying self-driving algorithms more efficiently. Recently, Neural Radiance Fields (NeRF) have been proposed for novel view synthesis using implicit reconstruction of 3D scenes. Inspired by this, we present NeRF-LIDAR, a novel LiDAR simulation method that leverages real-world information to generate realistic LIDAR point clouds. Different from existing LiDAR simulators, we use real images and point cloud data collected by self-driving cars to learn the 3D scene representation, point cloud generation and label rendering. We verify the effectiveness of our NeRF-LiDAR by training different 3D segmentation models on the generated LiDAR point clouds. It reveals that the trained models are able to achieve similar accuracy when compared with the same model trained on the real LiDAR data. Besides, the generated data is capable of boosting the accuracy through pre-training which helps reduce the requirements of the real labeled data.

==> fig_tex/3Dsegmentation.tex <==
\begin{figure*}
\centering


\begin{subfigure}[b]{0.485\linewidth}
\begin{minipage}[t]{1\linewidth}
\centering
\includegraphics[width=1\linewidth]
{figure/lidar_label1.png}
\includegraphics[width=1\linewidth]
{figure/lidar_label1.png}
%\caption{fig1}
\end{minipage}%
\caption{Our Data \& Label Rendering}
\end{subfigure}
\begin{subfigure}[b]{0.485\linewidth}
\begin{minipage}[t]{1\linewidth}
\centering
\includegraphics[width=1\linewidth]
{figure/lidar_label1.png}
\includegraphics[width=1\linewidth]
{figure/lidar_label1.png}
%\caption{fig1}
\end{minipage}%
\caption{Ground-truth Labels of the Real Data}
\end{subfigure}
\caption{Comparisons between the data and label generated by the NeRF-LiDAR and the real LiDAR data with human annotations. For better visualization, we project the 3D point cloud as 2D equirectangular image with colorized labels.  Our NeRF-LiDAR (a) is shown able to generate accurate labels and realistic point clouds that is almost the same as the real data (b).}
\label{fig:label_quality}
\end{figure*}

==> file/tables/ablation_scenes_num.tex <==
\setlength{\tabcolsep}{2.5pt}
\renewcommand\arraystretch{1.2}
\begin{table}[ht!] 
\setlength{\abovecaptionskip}{0pt}
\setlength{\belowcaptionskip}{-4pt}
%\vspace{-2mm}
\centering
\resizebox{1\linewidth}{!}{%
\large
\begin{tabular}{l|cccccc}
\toprule scenes number & road  & vege. & terrain & vehicle & manmade & mIoU\\
\midrule
25 scenes &91.6 &61.1& 59.2 &69.7& 68.0 &69.9\\
50 scenes & & &  & &  &\\
100 scenes  &93.9& 65.5& 65.7& 76.3 &73.5& 75.0\\

% \midrule
% Ours
% &  & &   \\
\bottomrule
\end{tabular}
}
\vspace{4mm}
\caption{Ablations on the scenes number. } 
%\label{tab:ablation}
\label{tab:ablation_scene_num}
 
\end{table}

==> file/tables/compare_timing.tex <==
\setlength{\tabcolsep}{2.5pt}
\renewcommand\arraystretch{1.2}
\begin{table}[t]

\centering
\resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|cc}
    \specialrule{.2em}{.2em}{.2em}
           & Training  & Rendering (per frame)\\ \hline
Urban-NeRF ~\cite{urban-nerf} & 24 hours  & 6s\\ 
PNF ~\cite{panoptic-neural}& $\sim$ 24 hours &$\sim$ 6s\\ 
NeRF-LiDAR &  1 hour & 0.3s\\ 
\specialrule{.2em}{.1em}{.1em}
    \end{tabular}
}
\vspace{0.5mm}
    \caption{Comparison of efficiency with other NeRFs}
    \label{tab:efficiency}
    \vspace{-4mm}
\end{table}

==> file/tables/supp_psnr_compare.tex <==
\setlength{\tabcolsep}{20pt}
\renewcommand\arraystretch{1.2}
\begin{table}[ht!]
\vspace{-1mm}
% \setlength{\abovecaptionskip}{2pt}
% \setlength{\belowcaptionskip}{-10pt}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|lll}
% &\multicolumn{3}{c|}{RGB metrics}  \\
\toprule
           & PSNR$\uparrow$ & SSIM $\uparrow$& LPIPS$\downarrow$ \\ \hline
NeRF-LiDAR &   \textbf{25.19 }  &  \textbf{0.802 }   &   \textbf{0.328}  \\ 
 %PNF\\
 Urban-NeRF ~\cite{urban-nerf} &21.12&	0.673	&0.503 \\
%\hline
           % &      &      &       &               &       
           \bottomrule
\end{tabular}
}
\vspace{1mm}
\caption{Evaluation of NeRF-LiDAR and Urban-NeRF using RGB metrics in the reconstructed scenes.}% Error rate∗\text{Error rate}^* means the percentage which of relative error exceeds 10%10\%}.
\label{tab:nerf_lidar_eva}
\end{table}
